A Cascaded Approach for ultraly High Performance Lesion Detection and False Positive Removal in Liver CT Scans

Liver cancer has high morbidity and mortality rates in the world. Multi-phase CT is a main medical imaging modality for detecting/identifying and diagnosing liver tumors. Automatically detecting and classifying liver lesions in CT images have the potential to improve the clinical workflow. This task remains challenging due to liver lesions' large variations in size, appearance, image contrast, and the complexities of tumor types or subtypes. In this work, we customize a multi-object labeling tool for multi-phase CT images, which is used to curate a large-scale dataset containing 1,631 patients with four-phase CT images, multi-organ masks, and multi-lesion (six major types of liver lesions confirmed by pathology) masks. We develop a two-stage liver lesion detection pipeline, where the high-sensitivity detecting algorithms in the first stage discover as many lesion proposals as possible, and the lesion-reclassification algorithms in the second stage remove as many false alarms as possible. The multi-sensitivity lesion detection algorithm maximizes the information utilization of the individual probability maps of segmentation, and the lesion-shuffle augmentation effectively explores the texture contrast between lesions and the liver. Independently tested on 331 patient cases, the proposed model achieves high sensitivity and specificity for malignancy classification in the multi-phase contrast-enhanced CT (99.2%, 97.1%, diagnosis setting) and in the noncontrast CT (97.3%, 95.7%, screening setting).

==> tables/AttentiveMultiROISensSpec.tex <==

\scriptsize

\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}T-score\\ Thresholds\end{tabular}} & \multicolumn{2}{c|}{L1} & \multicolumn{2}{c|}{L2} & \multicolumn{2}{c|}{L3} & \multicolumn{2}{c|}{L4} & \multicolumn{2}{c|}{Average} \\\cline{2-11}
& Sens       & Spec      & Sens       & Spec      & Sens       & Spec      & Sens       & Spec      & Sens         & Spec         \\\hline
-1.75                                                                         & 93.9\%     & 85.1\%    & 91.7\%     & 89.1\%    & 93.4\%     & 91.1\%    & 85.0\%     & 93.1\%    & 91.0\%       & 89.6\%       \\\hline
-2                                                                            & 86.2\%     & 91.0\%    & 85.0\%     & 93.0\%    & 84.8\%     & 94.8\%    & 75.4\%     & 95.4\%    & 82.8\%       & 93.6\%       \\\hline
-2.25                                                                         & 77.6\%     & 95.3\%    & 76.3\%     & 95.8\%    & 72.0\%     & 96.9\%    & 68.9\%     & 97.4\%    & 73.7\%       & 96.4\%       \\\hline
-2.5                                                                          & 61.9\%     & 97.5\%    & 63.5\%     & 97.9\%    & 60.7\%     & 98.3\%    & 54.5\%     & 98.9\%    & 60.2\%       & 98.1\%       \\\hline
Flex                                                                          & 79.8\%     & 94.7\%    & 82.3\%     & 94.4\%    & 84.8\%     & 94.8\%    & 78.4\%     & 94.4\%    & 81.3\%       & 94.6\% \\ \hline
\end{tabular}

% \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
% \hline
% \multirow{2}{*}{Threshold} & \multicolumn{2}{c|}{L1} & \multicolumn{2}{c|}{L2} & \multicolumn{2}{c|}{L3} & \multicolumn{2}{c|}{L4} & \multicolumn{2}{c|}{Avg} \\\cline{2-11} 
%                           & Sens.      & Spec.     & Sens.      & Spec.     & Sens.      & Spec.     & Sens.      & Spec.     & Sens.      & Spec.      \\\hline
% Tscore  -2.5               & 0.66       & 0.968     & 0.571      & 0.978     & 0.602      & 0.982     & 0.521      & 0.989     & 0.589     & 0.979    \\\hline
% Tscore  -1                 & 0.866      & 0.838     & 0.777      & 0.914     & 0.796      & 0.905     & 0.668      & 0.927     & 0.777    & 0.896     \\ \hline
% \end{tabular}


% \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
% \hline
% \multirow{}{}{Thres} & \multicolumn{4}{c|}{L1}        & \multicolumn{4}{c|}{L2}        & \multicolumn{4}{c|}{L3}        & \multicolumn{4}{c|}{L4}        \\ \hline
%                           & Sens  & Spec  & PosP  & NegP  & Sens  & Spec  & PosP  & NegP  & Sens  & Spec  & PosP  & NegP  & Sens  & Spec  & PosP  & NegP  \\ \hline
% T -2.5                       & 0.66  & 0.968 & 0.728 & 0.956 & 0.571 & 0.978 & 0.738 & 0.954 & 0.602 & 0.982 & 0.738 & 0.966 & 0.521 & 0.989 & 0.763 & 0.969 \\ \hline
% T -1                         & 0.866 & 0.838 & 0.836 & 0.867 & 0.777 & 0.914 & 0.857 & 0.862 & 0.796 & 0.905 & 0.81  & 0.898 & 0.668 & 0.927 & 0.793 & 0.869 \\ \hline
% L10\%                        & 0.648 & 0.97  & 0.732 & 0.956 & 0.63  & 0.979 & 0.818 & 0.947 & 0.634 & 0.974 & 0.767 & 0.951 & 0.556 & 0.972 & 0.759 & 0.933 \\ \hline
% L20\%                        & 0.728 & 0.948 & 0.796 & 0.926 & 0.709 & 0.963 & 0.859 & 0.912 & 0.715 & 0.957 & 0.835 & 0.917 & 0.63  & 0.94  & 0.774 & 0.886  \\ \hline
% \end{tabular}





==> tables/T390_base_lesion.tex <==
\scriptsize
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
gt, pred & HCC & Choln & Meta & Heman & Other & Cyst & Normal \\\cline{2-7}\hline
HCC      & 228 & 2     & 5    & 1     & 6     & 1    & 16     \\\hline
Choln    & 3   & 8     & 2    & 0     & 0     & 0    & 0      \\\hline
Meta     & 11  & 2     & 147  & 0     & 2     & 2    & 16     \\\hline
Heman    & 6   & 0     & 0    & 6     & 1     & 0    & 0      \\\hline
Other    & 16  & 1     & 7    & 1     & 31    & 0    & 5      \\\hline
Cyst     & 0   & 0     & 1    & 0     & 6     & 62   & 0      \\\hline
Normal   & 9   & 3     & 5    & 2     & 18    & 6    & 0      \\\hline

\end{tabular}

==> tables/T390_base_patient.tex <==
\scriptsize
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline

gt, pred & HCC & Choln & Meta & Heman & Other & Cyst & Normal \\\cline{2-7}\hline
HCC      & 201 & 4     & 6    & 1     & 1     & 0    & 3      \\\hline
Choln    & 2   & 8     & 2    & 0     & 0     & 0    & 0      \\\hline
Meta     & 7   & 2     & 23   & 0     & 1     & 0    & 0      \\\hline
Heman    & 2   & 0     & 0    & 4     & 0     & 0    & 0      \\\hline
Other    & 6   & 0     & 2    & 0     & 1     & 0    & 2      \\\hline
Cyst     & 0   & 0     & 0    & 0     & 0     & 2    & 0      \\\hline
Normal   & 2   & 2     & 1    & 0     & 2     & 1    & 43    \\\hline


\end{tabular}

==> tables/T390_gen20_lesion.tex <==
\scriptsize
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
gt, pred & HCC & Choln & Meta & Heman & Other & Cyst & Normal \\\cline{2-7}\hline
HCC      & 227 & 2     & 5    & 1     & 6     & 1    & 17     \\\hline
Choln    & 3   & 8     & 2    & 0     & 0     & 0    & 0      \\\hline
Meta     & 11  & 2     & 147  & 0     & 2     & 2    & 16     \\\hline
Heman    & 4   & 0     & 0    & 6     & 1     & 0    & 2      \\\hline
Other    & 14  & 1     & 7    & 2     & 26    & 0    & 11     \\\hline
Cyst     & 1   & 0     & 1    & 0     & 2     & 62   & 3      \\\hline
Normal   & 2   & 1     & 4    & 0     & 3     & 2    & 0     \\\hline

\end{tabular}

==> tables/T390_gen20_patient.tex <==
\scriptsize
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
gt, pred & HCC & Choln & Meta & Heman & Other & Cyst & Normal \\\cline{2-7}\hline
HCC      & 201 & 3     & 6    & 1     & 1     & 0    & 4      \\\hline
Choln    & 2   & 8     & 2    & 0     & 0     & 0    & 0      \\\hline
Meta     & 7   & 2     & 23   & 0     & 1     & 0    & 0      \\\hline
Heman    & 2   & 0     & 0    & 4     & 0     & 0    & 0      \\\hline
Other    & 6   & 0     & 1    & 0     & 1     & 0    & 3      \\\hline
Cyst     & 0   & 0     & 0    & 0     & 0     & 2    & 0      \\\hline
Normal   & 0   & 1     & 0    & 0     & 0     & 1    & 49    \\\hline

\end{tabular}

==> tables/T390_gen24_lesion.tex <==
\scriptsize
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
gt, pred & HCC & Choln & Meta & Heman & Other & Cyst & Normal \\\cline{2-7}\hline
HCC      & 232 & 2     & 4    & 1     & 6     & 2    & 11     \\\hline
Choln    & 3   & 8     & 2    & 0     & 0     & 0    & 0      \\\hline
Meta     & 11  & 2     & 135  & 0     & 2     & 1    & 13     \\\hline
Heman    & 4   & 0     & 0    & 6     & 1     & 0    & 2      \\\hline
Other    & 16  & 1     & 6    & 3     & 28    & 1    & 14     \\\hline
Cyst     & 0   & 0     & 2    & 0     & 1     & 63   & 7      \\\hline
Normal   & 9   & 1     & 10   & 1     & 10    & 4    & 0   \\\hline

\end{tabular}

==> tables/T390_gen24_patient.tex <==
\scriptsize
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
gt, pred & HCC & Choln & Meta & Heman & Other & Cyt & Nol \\\cline{2-7}\hline
HCC      & 209 & 2     & 4    & 0     & 0     & 0    & 1      \\\hline
Choln    & 2   & 8     & 2    & 0     & 0     & 0    & 0      \\\hline
Meta     & 7   & 2     & 23   & 0     & 1     & 0    & 0      \\\hline
Heman    & 2   & 0     & 0    & 4     & 0     & 0    & 0      \\\hline
Other    & 5   & 0     & 1    & 0     & 2     & 0    & 3      \\\hline
Cyst     & 0   & 0     & 0    & 0     & 0     & 1    & 1      \\\hline
Normal   & 1   & 1     & 0    & 0     & 1     & 1    & 47    \\\hline

\end{tabular}

==> tables/ablationEnsemble.tex <==
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
% \hline
% \multirow{2}{*}{Ensemble} & \multicolumn{2}{c|}{L1}         & \multicolumn{2}{c|}{L2}         & \multicolumn{2}{c|}{L3}         & \multicolumn{2}{c|}{L4}         & \multicolumn{2}{c|}{Average}    \\ \cline{2-11} 
%                           & R-value        & AUC            & R-value        & AUC            & R-value        & AUC            & R-value        & AUC            & R-value        & AUC            \\ \hline\hline
% Ensm\_roi             & 0.879          & 0.935          & 0.876          & 0.946          & 0.850          & 0.929          & 0.812          & 0.894          & 0.854          & 0.926          \\ \hline
% Ensm\_all             & \textbf{0.881} & \textbf{0.938} & \textbf{0.880} & \textbf{0.949} & \textbf{0.851} & \textbf{0.933} & \textbf{0.816} & \textbf{0.903} & \textbf{0.857} & \textbf{0.931} \\ \hline
% \end{tabular}

% \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
% \hline
% \multirow{2}{*}{Ensemble} & \multicolumn{2}{c|}{L1}         & \multicolumn{2}{c|}{L2}         & \multicolumn{2}{c|}{L3}         & \multicolumn{2}{c|}{L4}         & \multicolumn{2}{c|}{Average}    \\ \cline{2-11} 
%                           & R-value        & RMSE            & R-value        & RMSE            & R-value        & RMSE            & R-value        & RMSE            & R-value        & RMSE            \\ \hline\hline
% Base            & 0.879          & 0.11          & 0.876          & 0.134          & 0.850          & 0.129          & 0.812          & 0.139          & 0.854          & 0.128          \\ \hline
% All             & \textbf{0.888} & \textbf{0.102} & \textbf{0.886} & \textbf{0.108} & \textbf{0.869} & \textbf{0.125} & \textbf{0.815} & 0.141 & \textbf{0.864} & \textbf{0.119} \\ \hline
% \end{tabular}


\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{Ensemble} & \multicolumn{2}{c|}{L1}         & \multicolumn{2}{c|}{L2}         & \multicolumn{2}{c|}{L3}         & \multicolumn{2}{c|}{L4}         & \multicolumn{2}{c|}{Average}    \\ \cline{2-11} 
                          & R-value        & AUC            & R-value        & AUC            & R-value        & AUC            & R-value        & AUC            & R-value        & AUC            \\ \hline\hline
Bases            & 0.879          & 0.935          & 0.876          & 0.946          & 0.850          & 0.929          & 0.812          & 0.894          & 0.854          & 0.926          \\ \hline
All             & \textbf{0.888} & \textbf{0.947} & \textbf{0.886} & \textbf{0.954} & \textbf{0.869} & \textbf{0.939} & \textbf{0.815} & \textbf{0.907} & \textbf{0.864} & \textbf{0.937} \\ \hline
\end{tabular}


% Ensemble of 5 ROI models:
% 0.879	0.877	0.854	0.811	0.855
% 0.11	0.134	0.129	0.139	0.128
% roc_auc:  {0: 0.935, 1: 0.946, 2: 0.929, 3: 0.894, 'avg': 0.926}

% Ensemble of all 6 models: 
% 0.888	0.886	0.869	0.815	0.864
% 0.102	0.108	0.125	0.141	0.119
% roc_auc:  {0: 0.947, 1: 0.954, 2: 0.939, 3: 0.907, 'avg': 0.937}


==> tables/ablationFusion.tex <==
\scriptsize
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{Model} & \multicolumn{3}{c|}{L1} & \multicolumn{3}{c|}{L2} & \multicolumn{3}{c|}{L3} & \multicolumn{3}{c|}{L4} & \multicolumn{3}{c|}{Average} \\\cline{2-16} 
                       & R-Val  & RMSE  & AUC   & R-Val  & RMSE  & AUC   & R-Val  & RMSE  & AUC   & R-Val  & RMSE  & AUC   & R-Val   & RMSE    & AUC     \\\hline
Base                   & 0.859  & 0.089 & 0.952 & 0.87   & 0.101 & 0.96  & 0.86   & 0.104 & 0.966 & 0.823  & 0.12  & 0.963 & 0.853   & 0.104   & 0.96    \\\hline
MultiPatch             & 0.873  & 0.071 & 0.958 & 0.877  & 0.08  & 0.967 & 0.873  & 0.083 & 0.971 & 0.834  & 0.098 & 0.965 & 0.864   & 0.083   & 0.965   \\\hline
AttMultiPatch          & 0.885          & 0.068          & 0.964          & 0.888          & 0.076          & \textbf{0.967} & 0.882          & 0.081          & 0.969          & 0.846          & 0.094          & 0.964          & 0.875          & 0.08           & 0.966          \\\hline
MultiROI               & 0.883  & 0.068 & 0.959 & 0.887  & 0.076 & 0.966 & 0.879  & 0.082 & 0.972 & 0.837  & 0.097 & 0.966 & 0.871   & 0.081   & 0.966   \\\hline
\textbf{Proposed}      & \textbf{0.894} & \textbf{0.065} & \textbf{0.964} & \textbf{0.899} & \textbf{0.073} & 0.966          & \textbf{0.887} & \textbf{0.079} & \textbf{0.972} & \textbf{0.855} & \textbf{0.092} & \textbf{0.968} & \textbf{0.884} & \textbf{0.077} & \textbf{0.968} \\\hline
\end{tabular}

% \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
% \hline
% \multirow{2}{*}{Model} & \multicolumn{3}{c|}{L1}                           & \multicolumn{3}{c|}{L2}                                                           & \multicolumn{3}{c|}{L3}                                                           & \multicolumn{3}{c|}{L4}                                                           & \multicolumn{3}{c|}{Avg}                          \\\cline{2-16} 
%                       & R-Val        & RMSE           & AUC            & \multicolumn{1}{c|}{R-val} & \multicolumn{1}{c|}{RMSE} & \multicolumn{1}{c|}{AUC} & \multicolumn{1}{c|}{R-val} & \multicolumn{1}{c|}{RMSE} & \multicolumn{1}{c|}{AUC} & \multicolumn{1}{c|}{R-val} & \multicolumn{1}{c|}{RMSE} & \multicolumn{1}{c|}{AUC} & R-val        & RMSE           & AUC            \\\hline
% Baseline               & 0.866          & 0.074          & 0.956          & 0.870                       & 0.083                    & 0.959                   & 0.863                       & 0.086                    & 0.966                   & 0.822                       & 0.103                    & 0.959                   & 0.855          & 0.086          & 0.960          \\\hline
% MulPat                 & 0.872          & 0.071          & 0.960          & 0.880                       & 0.079                    & \textbf{0.966}          & 0.874                       & 0.083                    & 0.970                   & 0.834                       & 0.096                    & 0.963                   & 0.865          & 0.082          & 0.965         \\\hline
% AttMulPat              & 0.879          & 0.070          & 0.961          & 0.882                       & 0.078                    & 0.964                   & 0.873                       & 0.083                    & 0.967                   & 0.838                       & 0.096                    & 0.961                   & 0.868          & 0.081          & 0.963          \\\hline

% MulRoi                 & 0.883          & 0.068          & 0.961          & 0.887                       & 0.077                    & 0.965                   & 0.877                       & \textbf{0.082}           & \textbf{0.971}          & 0.838                       & 0.096                    & 0.960                   & 0.871          & 0.081          & 0.964          \\\hline
% \textbf{Ours}              & \textbf{0.889} & \textbf{0.067} & \textbf{0.963} & \textbf{0.889}              & \textbf{0.076}           & 0.964                   & \textbf{0.878}              & \textbf{0.082}           & \textbf{0.971}          & \textbf{0.840}              & \textbf{0.095}           & \textbf{0.966}          & \textbf{0.874} & \textbf{0.080} & \textbf{0.966} \\\hline
% \end{tabular}

==> tables/ablation_sexage.tex <==
\scriptsize
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{Patch} & \multicolumn{3}{c|}{L1}                           & \multicolumn{3}{c|}{L2}                                                           & \multicolumn{3}{c|}{L3}                                                           & \multicolumn{3}{c|}{L4}                                                           & \multicolumn{3}{c|}{Avg}                          \\\cline{2-16} 
                       & R-Val        & RMSE           & AUC            & \multicolumn{1}{c|}{R-val} & \multicolumn{1}{c|}{RMSE} & \multicolumn{1}{c|}{AUC} & \multicolumn{1}{c|}{R-val} & \multicolumn{1}{c|}{RMSE} & \multicolumn{1}{c|}{AUC} & \multicolumn{1}{c|}{R-val} & \multicolumn{1}{c|}{RMSE} & \multicolumn{1}{c|}{AUC} & R-val        & RMSE           & AUC            \\\hline
All & 0.888  & 0.067 & 0.963 & 0.889  & 0.076 & 0.964 & 0.878  & 0.082 & 0.971 & 0.840  & 0.095 & 0.966 & 0.874  & 0.080  & 0.966 \\\hline
M40-50                      & 0.845  & 0.067 & 0.980 & 0.848  & 0.076 & 0.992 & 0.842  & 0.080 & 0.990 & 0.822  & 0.085 & 0.947 & 0.839  & 0.077  & 0.977 \\\hline
M50-60                      & 0.866  & 0.065 & 0.940 & 0.857  & 0.076 & 0.926 & 0.844  & 0.080 & 0.955 & 0.801  & 0.094 & 0.955 & 0.842  & 0.079  & 0.944 \\\hline
M60-70                      & 0.820  & 0.077 & 0.978 & 0.795  & 0.089 & 0.972 & 0.779  & 0.101 & 0.922 & 0.726  & 0.116 & 0.994 & 0.780  & 0.095  & 0.966 \\\hline
M70-90                      & 0.884  & 0.077 & 0.980 & 0.876  & 0.091 & 0.977 & 0.851  & 0.103 & 0.966 & 0.833  & 0.115 & 0.953 & 0.861  & 0.096  & 0.969 \\\hline
F40-50                      & 0.871  & 0.060 & 0.970 & 0.866  & 0.068 & 0.983 & 0.870  & 0.070 & 0.997 & 0.838  & 0.083 & 0.978 & 0.861  & 0.070  & 0.982 \\\hline
F50-60                      & 0.897  & 0.060 & 0.946 & 0.904  & 0.064 & 0.948 & 0.896  & 0.071 & 0.958 & 0.864  & 0.085 & 0.943 & 0.890  & 0.070  & 0.949 \\\hline
F60-70                      & 0.882  & 0.065 & 0.931 & 0.889  & 0.074 & 0.932 & 0.886  & 0.080 & 0.936 & 0.820  & 0.104 & 0.926 & 0.869  & 0.081  & 0.931 \\\hline
F70-90                      & 0.798  & 0.093 & 0.873 & 0.777  & 0.098 & 0.878 & 0.805  & 0.106 & 0.883 & 0.777  & 0.120 & 0.912 & 0.789  & 0.104  & 0.886
       
  \\\hline
\end{tabular}


% \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
% \hline
% \multirow{}{}{Data} & \multicolumn{3}{c|}{L1}                              & \multicolumn{3}{c|}{L2}                                                           & \multicolumn{3}{c|}{L3}                                                           & \multicolumn{3}{c|}{L4}
%             & \multicolumn{1}{c|}{train}& \multicolumn{1}{c|}{test}
% \\ \cline{2-13} 
% Range & R-value & RMSE   & AUC    & R-value & RMSE   & AUC    & R-value & RMSE   & AUC    & R-value & RMSE   & AUC    & \multirow{}{}{\#} & \multirow{}{}{\#} \\ \hline 
% All  & 0.8885  & 0.0669  & 0.9626 & 0.8892  & 0.0757 & 0.9644 & 0.8776  & 0.0815 & 0.9713 & 0.8399   & 0.0954 & 0.9658 & 11024                      & 2695                      \\ \hline  \hline
% M40-50                       & 0.8454  & 0.0673 & 0.9802 & 0.848   & 0.0755 & 0.9915 & 0.842   & 0.0796 & 0.9895 & 0.822   & 0.0849 & 0.9473 & 1605                       & 372                       \\ \hline
% M50-60                       & 0.8663  & 0.0651 & 0.9396 & 0.8567  & 0.0759 & 0.9259 & 0.8437  & 0.0799 & 0.955  & 0.8012  & 0.0943 & 0.9545 & 2095                       & 499                       \\ \hline
% M60-70                       & 0.8196  & 0.0766 & 0.9776 & 0.7953  & 0.089  & 0.9719 & 0.7792  & 0.1006 & 0.9218 & 0.7261  & 0.1156 & 0.9943 & 1258                       & 292                       \\ \hline
% M70-90                       & 0.8836  & 0.0768 & 0.9796 & 0.876   & 0.0912 & 0.9765 & 0.8509  & 0.1027 & 0.966  & 0.8328  & 0.1149 & 0.9532 & 468                        & 123                       \\ \hline
% F40-50                       & 0.8705  & 0.0599 & 0.9703 & 0.8657  & 0.0678 & 0.9833 & 0.8695  & 0.0699 & 0.9967 & 0.8378  & 0.0829 & 0.9784 & 1589                       & 435                       \\ \hline
% F50-60                       & 0.8966  & 0.0596 & 0.9457 & 0.904   & 0.0638 & 0.948  & 0.8956  & 0.0713 & 0.9581 & 0.8637  & 0.0848 & 0.9432 & 2279                       & 564                       \\ \hline
% F60-70                       & 0.8823  & 0.0646 & 0.931  & 0.8891  & 0.0743 & 0.9318 & 0.8859  & 0.0797 & 0.9356 & 0.8199  & 0.1044 & 0.9259 & 1205                       & 277                       \\ \hline
% F70-90                       & 0.7981  & 0.0926 & 0.8731 & 0.7766  & 0.0981 & 0.8777 & 0.8051  & 0.1058 & 0.8831 & 0.7769  & 0.1202 & 0.9119 & 525                        & 133                      

%       \\ \hline
% \end{tabular}


==> tables/backupTables.tex <==
%%% lesion statistics
\scriptsize
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
Volume & 0.5$\sim$2 & 2$\sim$4 &4$\sim$8& 8$\sim$16 & 16$\sim$64 & $>$64 & Total & Cases \\\hline\hline
HCC    & 22         & 28       & 36       & 47        & 60         & 66               & 259 & 216   \\\hline
Choln  & 0          & 0        & 1        & 2         & 7          & 3                & 13  & 13    \\\hline
Meta   & 69         & 27       & 32       & 18        & 24         & 22               & 192 & 34    \\\hline
Hem  & 1          & 2        & 1        & 0         & 3          & 5                & 12  & 8     \\\hline
Other  & 25         & 8        & 7        & 11        & 8          & 2                & 61  & 46    \\\hline
Cyst   & 51         & 7        & 8        & 1         & 2          & 0                & 69  & 46    \\\hline
\textbf{All}    & 168        & 72       & 85       & 79        & 104        & 98               & 606 & 280  \\\hline
\textbf{Malig}  & 91         & 55       & 69       & 67        & 91         & 91               & 464 & 261   \\\hline
\end{tabular}

%%% patient-level: four-phase, NC-phase
\scriptsize
\begin{tabular}{|c|c|c|c|c|c|c||c|c|c|c|c|c|}
\hline
Dataset setting & \multicolumn{6}{c||}{Four phase}  & \multicolumn{6}{c|}{NC phase} \\\hline
\multirow{2}{*}{Model \textbackslash Metrics} & \multicolumn{2}{c|}{All} & \multicolumn{4}{c||}{Malignancy}    & \multicolumn{2}{c|}{All} & \multicolumn{4}{c|}{Malignancy}    \\\cline{2-13}
                                                & Accu       & L.Accu     & Preci  & Sens   & Spec   & F      & Accu       & L.Accu     & Preci  & Sens   & Spec   & F      \\\hline
Sens1 w/o Patch                               & 85.2\%     & 92.4\%     & 98.1\% & 97.7\% & 92.9\% & 97.9\% & 81.3\%     & 88.2\%     & 95.4\% & 95.0\% & 82.9\% & 95.2\% \\\hline
Sens1 w. Patch (no CA)                        & 86.1\%     & 93.1\%     & 99.6\% & 96.2\% & 98.6\% & 97.9\% & 80.1\%     & 87.0\%     & 99.6\% & 89.3\% & 98.6\% & 94.2\% \\\hline
Sens1 w. Patch                                  & 87.0\%     & 94.0\%     & 99.6\% & 97.3\% & 98.6\% & 98.4\% & 81.6\%     & 88.8\%     & 98.8\% & 92.3\% & 95.7\% & 95.4\% \\\hline
Sens4 w. Patch                                  & 88.8\%     & 95.2\%     & 99.2\% & 99.2\% & 97.1\% & 99.2\% & 84.3\%     & 92.4\%     & 98.8\% & 97.3\% & 95.7\% & 98.0\% \\\hline
Sens1 w. Patch   + Sens4 w. Patch               & 89.3\%     & 95.6\%     & 99.6\% & 99.2\% & 98.5\% & 99.4\% & 86.6\%     & 93.8\%     & 99.6\% & 97.5\% & 98.4\% & 98.5\% \\\hline
\end{tabular}

%%% liver main table
\scriptsize

\begin{tabular}{|c|c|c|c|c||c|c|c|c|}
\hline
\multirow{2}{*}{Model \textbackslash Scene Metrics}  & \multicolumn{4}{c||}{$Diagnosis$ of \textbf{Malig}}  &  \multicolumn{4}{c|}{$Screening$ of \textbf{Malig}}  \\\cline{2-9}
                                                  & \textit{Preci}  & \textit{Sens}   & \textit{Spec}   & \textit{F}     & \textit{Preci}  & \textit{Sens}   & \textit{Spec}   & \textit{F}      \\\hline
\textit{Base}                         & 98.1\% & 97.7\% & 92.9\% & 97.9\%      & 95.4\% & 95.0\% & 82.9\% & 95.2\% \\\hline
\textit{Base+ReCls w/o LS}              & 99.6\% & 96.2\% & 98.6\% & 97.9\%      & 99.6\% & 89.3\% & 98.6\% & 94.2\% \\\hline
\textit{Base+ReCls}                         & 99.6\% & 97.3\% & 98.6\% & 98.4\%      & 98.8\% & 92.3\% & 95.7\% & 95.4\% \\\hline
\textit{High+ReCls}                          & 99.2\% & 99.2\% & 97.1\% & 99.2\%      & 98.8\% & 97.3\% & 95.7\% & 98.0\% \\\hline
\textit{Base+Recls \& High+ReCls}       & 99.6\% & 99.2\% & 98.5\% & 99.4\%      & 99.6\% & 97.5\% & 98.4\% & 98.5\% \\\hline

\end{tabular}




==> tables/baseline_backbones.tex <==

\scriptsize
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{Backbone} & \multicolumn{3}{c|}{L1}                           & \multicolumn{3}{c|}{L2}                                                           & \multicolumn{3}{c|}{L3}                                                           & \multicolumn{3}{c|}{L4}                                                           & \multicolumn{3}{c|}{Avg}                          \\\cline{2-16} 
                       & R-Val        & RMSE           & AUC            & \multicolumn{1}{c|}{R-val} & \multicolumn{1}{c|}{RMSE} & \multicolumn{1}{c|}{AUC} & \multicolumn{1}{c|}{R-val} & \multicolumn{1}{c|}{RMSE} & \multicolumn{1}{c|}{AUC} & \multicolumn{1}{c|}{R-val} & \multicolumn{1}{c|}{RMSE} & \multicolumn{1}{c|}{AUC} & R-val        & RMSE           & AUC            \\\hline
VGG13                     & 0.864          & 0.075          & 0.954          & 0.865          & 0.084          & 0.956          & 0.862          & 0.088          & 0.965          & \textbf{0.828} & 0.099          & 0.957          & 0.855 & 0.086          & 0.958          \\\hline
VGG16                     & \textbf{0.866} & \textbf{0.074} & \textbf{0.956} & \textbf{0.870} & 0.083          & 0.959          & \textbf{0.863} & \textbf{0.086} & \textbf{0.966} & 0.822          & 0.103          & 0.959          & \textbf{0.855} & 0.086          & \textbf{0.960} \\\hline
VGG19                     & 0.863          & 0.075          & 0.955          & \textbf{0.870} & \textbf{0.082} & 0.958          & 0.861          & 0.087          & 0.961          & 0.824          & \textbf{0.098} & \textbf{0.960} & 0.855 & \textbf{0.085} & 0.958          \\\hline
ResN18                    & 0.831          & 0.082          & 0.943          & 0.846          & 0.093          & 0.955          & 0.835          & 0.095          & 0.953          & 0.794          & 0.106          & 0.953          & 0.826          & 0.094          & 0.951          \\\hline
ResN34                    & 0.845          & 0.078          & 0.948          & 0.851          & 0.088          & 0.957          & 0.843          & 0.092          & \textbf{0.966} & 0.804          & 0.105          & 0.953          & 0.836          & 0.091          & 0.956          \\\hline
ResN50                    & 0.852          & 0.078          & 0.949          & 0.857          & 0.085          & \textbf{0.961} & 0.852          & 0.092          & 0.964          & 0.814          & 0.104          & 0.957          & 0.844          & 0.090          & 0.958          \\\hline
ResN101                   & 0.846          & 0.078          & 0.949          & 0.860          & 0.087          & 0.959          & 0.855          & 0.090          & 0.965          & 0.805          & 0.105          & 0.955          & 0.841          & 0.090          & 0.957         
  \\\hline
\end{tabular}



% \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|}
% \hline
% \multirow{2}{*}{Baseline} & \multicolumn{3}{c|}{L1}                              & \multicolumn{3}{c|}{L2}                                                           & \multicolumn{3}{c|}{L3}                                                           & \multicolumn{3}{c|}{L4}                                                           \\ \cline{2-13} 
%       & R-value   & RMSE   & AUC   & R-value & RMSE  & AUC & R-value   & RMSE  & AUC & R-value    & RMSE   & AUC \\ \hline\hline
% VGG13                              & 0.8638          & 0.0748          & 0.9541          & 0.8647          & 0.0835         & 0.9563          & 0.8616          & 0.0877          & 0.9651          & 0.8281          & 0.0994          & 0.9565          \\ \hline
% VGG16                              & \textbf{0.8661} & \textbf{0.0744} & \textbf{0.9557} & 0.8696          & 0.0825         & 0.9585          & \textbf{0.8625} & \textbf{0.0863} & 0.9655          & 0.8222          & 0.1025          & 0.9586          \\ \hline
% VGG19                              & 0.8632          & 0.0745          & 0.9547          & \textbf{0.8702} & \textbf{0.082} & 0.9581          & 0.8613          & 0.0869          & 0.9606          & \textbf{0.8289} & \textbf{0.0983} & \textbf{0.9596} \\ \hline
% Resnet18                           & 0.8306          & 0.0818          & 0.9434          & 0.8461          & 0.0927         & 0.9548          & 0.8349          & 0.0949          & 0.9531          & 0.7939          & 0.1062          & 0.9526          \\ \hline
% Resnet34                           & 0.8445          & 0.0783          & 0.9478          & 0.8507          & 0.0879         & 0.9573          & 0.8429          & 0.0921          & \textbf{0.9658} & 0.8044          & 0.1054          & 0.9529          \\ \hline
% Resnet50                           & 0.8519          & 0.0781          & 0.9487          & 0.8566          & 0.0853         & \textbf{0.9606} & 0.8522          & 0.092           & 0.9643          & 0.8136          & 0.1043          & 0.957           \\ \hline 
% Resnet101                          & 0.8461          & 0.0775          & 0.9493          & 0.8597          & 0.0873         & 0.9586          & 0.8551          & 0.09            & 0.9649          & 0.8049          & 0.1046          & 0.9554         

%       \\ \hline
% \end{tabular}


==> tables/data_analyze_RMSE.tex <==

\begin{tabular}{|c||c|c|c|c|}
\hline
RMSE & L1     & L2     & L3     & L4     \\\hline\hline
L1   & 0.000 & 0.101 & 0.177 & 0.192 \\\hline
L2   & 0.101 & 0.000 & 0.101 & 0.129 \\\hline
L3   & 0.177 & 0.101 & 0.000 & 0.079 \\\hline
L4   & 0.192 & 0.129 & 0.079 & 0.000 \\\hline
\end{tabular}


==> tables/data_analyze_Rvalue.tex <==

\begin{tabular}{|c||c|c|c|c|}
\hline
R-values & L1     & L2     & L3     & L4     \\ \hline\hline
L1       & 1.000 & 0.918 & 0.878 & 0.807 \\\hline
L2       & 0.918 & 1.000 & 0.931 & 0.836 \\\hline
L3       & 0.878 & 0.931 & 1.000 & 0.898 \\\hline
L4       & 0.807 & 0.836 & 0.898 & 1.000 \\\hline
\end{tabular}


==> tables/liver_final_lesion_level_1phase.tex <==
\scriptsize
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{Type \textbackslash Metrics} & \multicolumn{7}{c|}{\textit{High+ReCls}} \\\cline{2-8}
                                          & \textit{FN}   & \textit{FP}   & \textit{FL}   & \textit{TP}    & \textit{Preci}    & \textit{Recal}     & \textit{Recal.bin}      \\\hline
HCC                                       & 18   & 9    & 9    & 207   & 77.2\%   & 88.5\%  & 92.3\%   \\\hline
ICC                                     & 0    & 1    & 9    & 4     & 50.0\%   & 30.8\%  & 100.0\%  \\\hline
Meta                                      & 16   & 10   & 27   & 89    & 84.8\%   & 67.4\%  & 87.9\%   \\\hline
Hem                                     & 1    & 0    & 5    & 3     & 100.0\%  & 33.3\%  & 88.9\%   \\\hline
Other                                     & 10   & 4    & 22   & 19    & 67.9\%   & 37.3\%  & 80.4\%   \\\hline
Cyst                                      & 2    & 4    & 1    & 57    & 83.8\%   & 95.0\%  & 96.7\%   \\\hline
\textbf{All}                                       & 47   & 28   & 73   & 379   & 79.0\%   & 76.0\%  & 90.6\%   \\\hline
\textbf{Malig}                                     & 34   & 20   & 11   & 334   & 94.4\%   & 88.1\%  & 91.0\%  \\\hline

\end{tabular}

==> tables/liver_final_patient_level_1phase.tex <==
\scriptsize
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{GT \textbackslash Pred} & \multicolumn{7}{c|}{NC phase: Sens1 w. Patch + Sens4 w. Patch (305 cases)} \\\cline{2-8}
                         & FN     & FP     & FL     & TP      & Preci       & Sens       & Spec       \\\hline
HCC                      & 3      & 0      & 7      & 193     & 89.4\%      & 95.1\%     & 100.0\%    \\\hline
Choln                    & 0      & 1      & 8      & 4       & 57.1\%      & 33.3\%     & 99.7\%     \\\hline
Meta                     & 0      & 0      & 10     & 19      & 76.0\%      & 65.5\%     & 100.0\%    \\\hline
Heman                    & 0      & 0      & 2      & 2       & 100.0\%     & 50.0\%     & 100.0\%    \\\hline
Other                    & 3      & 0      & 7      & 0       & 0.0\%       & 0.0\%      & 100.0\%    \\\hline
Cyst                     & 0      & 0      & 0      & 1       & 50.0\%      & 100.0\%    & 100.0\%    \\\hline
All                      & 6      & 1      & 34     & 219     & 86.2\%      & 84.6\%     & 97.8\%     \\\hline
Malig                    & 3      & 1      & 3      & 238     & 99.6\%      & 97.5\%     & 98.4\%    \\\hline

\end{tabular}

==> tables/liver_final_patient_level_4phase.tex <==
\scriptsize
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{GT \textbackslash Pred} & \multicolumn{7}{c|}{Four phase: Sens1 w. Patch + Sens4 w. Patch (319 cases)} \\\cline{2-8}
                         & FN     & FP     & FL     & TP      & Preci       & Sens       & Spec       \\\hline
HCC                      & 1      & 0      & 6      & 201     & 92.6\%      & 96.6\%      & 100.0\%     \\\hline
Choln                    & 0      & 1      & 4      & 8       & 61.5\%      & 66.7\%      & 99.7\%      \\\hline
Meta                     & 0      & 0      & 10     & 23      & 76.7\%      & 69.7\%      & 100.0\%     \\\hline
Heman                    & 0      & 0      & 2      & 4       & 100.0\%     & 66.7\%      & 100.0\%     \\\hline
Other                    & 3      & 0      & 6      & 1       & 50.0\%      & 10.0\%      & 100.0\%     \\\hline
Cyst                     & 0      & 1      & 0      & 1       & 50.0\%      & 100.0\%     & 99.7\%      \\\hline
All                      & 4      & 2      & 28     & 238     & 88.8\%      & 88.1\%      & 95.9\%      \\\hline
Malig                    & 1      & 1      & 1      & 251     & 99.6\%      & 99.2\%      & 98.5\%   \\\hline

\end{tabular}

==> tables/liver_final_patient_level_4phase_1phase.tex <==
\scriptsize
\begin{tabular}{|c|c|c|c|c|c|c|c||c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{GT \textbackslash Pred} & \multicolumn{7}{c||}{Four phase: Sens1 w. Patch + Sens4 w. Patch (319 cases)} & \multicolumn{7}{c|}{NC phase: Sens1 w. Patch + Sens4 w. Patch (305 cases)} \\\cline{2-14}
                         & FN     & FP     & FL     & TP      & Preci       & Sens        & Spec        & FN     & FP     & FL     & TP      & Preci       & Sens        & Spec        \\\hline
HCC                      & 1      & 0      & 6      & 201     & 92.6\%      & 96.6\%      & 100.0\%     & 3      & 0      & 7      & 193     & 89.4\%      & 95.1\%      & 100.0\%     \\\hline
Choln                    & 0      & 1      & 4      & 8       & 61.5\%      & 66.7\%      & 99.7\%      & 0      & 1      & 8      & 4       & 57.1\%      & 33.3\%      & 99.7\%      \\\hline
Meta                     & 0      & 0      & 10     & 23      & 76.7\%      & 69.7\%      & 100.0\%     & 0      & 0      & 10     & 19      & 76.0\%      & 65.5\%      & 100.0\%     \\\hline
Heman                    & 0      & 0      & 2      & 4       & 100.0\%     & 66.7\%      & 100.0\%     & 0      & 0      & 2      & 2       & 100.0\%     & 50.0\%      & 100.0\%     \\\hline
Other                    & 3      & 0      & 6      & 1       & 50.0\%      & 10.0\%      & 100.0\%     & 3      & 0      & 7      & 0       & 0.0\%       & 0.0\%       & 100.0\%     \\\hline
Cyst                     & 0      & 1      & 0      & 1       & 50.0\%      & 100.0\%     & 99.7\%      & 0      & 0      & 0      & 1       & 50.0\%      & 100.0\%     & 100.0\%     \\\hline
All                      & 4      & 2      & 28     & 238     & 88.8\%      & 88.1\%      & 95.9\%      & 6      & 1      & 34     & 219     & 86.2\%      & 84.6\%      & 97.8\%      \\\hline
Malig                    & 1      & 1      & 1      & 251     & 99.6\%      & 99.2\%      & 98.5\%      & 3      & 1      & 3      & 238     & 99.6\%      & 97.5\%      & 98.4\%     \\\hline

\end{tabular}

==> tables/liver_final_patient_level_category_4phase_1phase.tex <==
\scriptsize

\begin{tabular}{|c|c|c|c|c||c|c|c|c|}
\hline
\multirow{2}{*}{GT\textbackslash Pred} & \multicolumn{4}{c||}{Four phase: proposed model} & \multicolumn{4}{c|}{NC phase: proposed model} \\\cline{2-9}
                                          & Malig     & Beni    & Norm    & Uctn    & Malig    & Beni    & Norm    & Uctn   \\\hline
Malig                                     & 251       & 1         & 1         & 8            & 238      & 3         & 3         & 17          \\\hline
Beni                                    & 8         & 6         & 3         & 2            & 9        & 3         & 3         & 4           \\\hline
Norm                                    & 1         & 1         & 47        & 2            & 1        & 0         & 45        & 5       \\\hline   

\end{tabular}

==> tables/liver_result_patientLevel_joint.tex <==
\scriptsize
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
gt, pred & HCC & Choln & Meta & Heman & Other & Cyst & Normal \\\cline{2-7}\hline
HCC      & 201 & 2     & 4    & 0     & 0     & 0    & 1      \\\hline
Choln    & 2   & 8     & 2    & 0     & 0     & 0    & 0      \\\hline
Meta     & 7   & 2     & 23   & 0     & 1     & 0    & 0      \\\hline
Heman    & 2   & 0     & 0    & 4     & 0     & 0    & 0      \\\hline
Other    & 5   & 0     & 1    & 0     & 1     & 0    & 3      \\\hline
Cyst     & 0   & 0     & 0    & 0     & 0     & 1    & 0      \\\hline
Normal   & 0   & 1     & 0    & 0     & 0     & 1    & 47    \\\hline
\end{tabular}


==> tables/mainRvalMaeAuc.tex <==
\scriptsize
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{Model} & \multicolumn{3}{c|}{L1} & \multicolumn{3}{c|}{L2} & \multicolumn{3}{c|}{L3} & \multicolumn{3}{c|}{L4} & \multicolumn{3}{c|}{Average} \\\cline{2-16} 
                       & R-Val  & MAE  & AUC   & R-Val  & MAE  & AUC   & R-Val  & MAE  & AUC   & R-Val  & MAE  & AUC   & R-Val   & MAE$\pm$SD    & AUC     \\\hline
Base                                       & 0.859                     & 0.069                   & 0.952                   & 0.87                      & 0.078                   & 0.96                    & 0.86                      & 0.08                    & 0.966                   & 0.823                     & 0.091                   & 0.963                   & 0.853                     & 0.08$\pm$0.066                    & 0.96                    \\\hline
MultiPatch                                 & 0.873                     & 0.054                   & 0.958                   & 0.877                     & 0.061                   & 0.967                   & 0.873                     & 0.063                   & 0.971                   & 0.834                     & 0.075                   & 0.965                   & 0.864                     & 0.063$\pm$0.053                   & 0.965                   \\\hline
AttMultiPatch                              & 0.885                     & 0.052                   & 0.964                   & 0.888                     & 0.059                   & \textbf{0.967}                   & 0.882                     & 0.061                   & 0.969                   & 0.846                     & 0.072                   & 0.964                   & 0.875                     & 0.061$\pm$0.051                   & 0.966                   \\\hline
MultiROI                                   & 0.883                     & 0.052                   & 0.959                   & 0.887                     & 0.059                   & 0.966                   & 0.879                     & 0.062                   & 0.972                   & 0.837                     & 0.074                   & 0.966                   & 0.871                     & 0.062$\pm$0.052                   & 0.966                   \\\hline
\textbf{Proposed}                          & \textbf{0.894}            & \textbf{0.049}          & \textbf{0.964}          & \textbf{0.899}            & \textbf{0.055}          & 0.966          & \textbf{0.887}            & \textbf{0.059}          & \textbf{0.972}          & \textbf{0.855}            & \textbf{0.069}          & \textbf{0.968}          & \textbf{0.884}            & \textbf{0.058$\pm$0.05}          & \textbf{0.968}         
 \\\hline
\end{tabular}

==> tables/multiPatchDim.tex <==


\scriptsize
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{Patch} & \multicolumn{3}{c|}{L1}                           & \multicolumn{3}{c|}{L2}                                                           & \multicolumn{3}{c|}{L3}                                                           & \multicolumn{3}{c|}{L4}                                                           & \multicolumn{3}{c|}{Avg}                          \\\cline{2-16} 
                       & R-Val        & RMSE           & AUC            & \multicolumn{1}{c|}{R-val} & \multicolumn{1}{c|}{RMSE} & \multicolumn{1}{c|}{AUC} & \multicolumn{1}{c|}{R-val} & \multicolumn{1}{c|}{RMSE} & \multicolumn{1}{c|}{AUC} & \multicolumn{1}{c|}{R-val} & \multicolumn{1}{c|}{RMSE} & \multicolumn{1}{c|}{AUC} & R-val        & RMSE           & AUC            \\\hline
2 x 2                      & 0.861          & 0.075          & 0.954          & 0.868          & 0.082          & 0.962          & 0.858          & 0.088          & 0.965          & 0.821          & 0.100          & 0.960          & 0.852          & 0.086          & 0.960          \\\hline
3 x 3                     & 0.872 & 0.071 & 0.960 & 0.880 & 0.079 & \textbf{0.966} & 0.874 & 0.083 & 0.970 & 0.834          & 0.096          & 0.963          & 0.865 & 0.082 & 0.965 \\\hline
4 x 4                      & 0.867          & 0.073          & 0.956          & 0.876          & 0.080          & 0.964          & 0.867          & 0.085          & 0.966          & 0.836 & 0.096 & 0.966 & 0.861          & 0.083          & 0.963         
  \\\hline
\textbf{Ours}              & \textbf{0.889} & \textbf{0.067} & \textbf{0.963} & \textbf{0.889}              & \textbf{0.076}           & 0.964                   & \textbf{0.878}              & \textbf{0.082}           & \textbf{0.971}          & \textbf{0.840}              & \textbf{0.095}           & \textbf{0.966}          & \textbf{0.874} & \textbf{0.080} & \textbf{0.966} \\\hline


\end{tabular}







% \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|}
% \hline
% \multirow{2}{*}{Multi-Patch} & \multicolumn{3}{c|}{L1}                              & \multicolumn{3}{c|}{L2}                                                           & \multicolumn{3}{c|}{L3}                                                           & \multicolumn{3}{c|}{L4}                                                           \\ \cline{2-13} 
%       & R-value   & RMSE   & AUC   & R-value & RMSE  & AUC & R-value   & RMSE  & AUC & R-value    & RMSE   & AUC \\ \hline\hline
% 2 * 2                                                                        & 0.8606          & 0.0747          & 0.9538          & 0.8683          & 0.0823          & 0.962           & 0.8583          & 0.0877          & 0.9651          & 0.821           & 0.0998          & 0.9601          \\ \hline
% 3 * 3                                                                        & \textbf{0.8719} & \textbf{0.0707} & \textbf{0.9603} & \textbf{0.8803} & \textbf{0.0787} & \textbf{0.9658} & \textbf{0.8735} & \textbf{0.0825} & \textbf{0.9697} & 0.8344          & 0.0964          & 0.9628          \\ \hline
% 4 * 4                                                                        & 0.8666          & 0.0728          & 0.9564          & 0.8762          & 0.0797          & 0.9637          & 0.8668          & 0.0845          & 0.9659          & \textbf{0.8357} & \textbf{0.0959} & \textbf{0.9658}
%       \\ \hline
% \end{tabular}



==> tables/networkComparison.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}

\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{Backbone} & \multicolumn{2}{c|}{L1}         & \multicolumn{2}{c|}{L2}         & \multicolumn{2}{c|}{L3}         & \multicolumn{2}{c|}{L4}         & \multicolumn{2}{c|}{Average}    \\ \cline{2-11} 
                          & R-value        & AUC            & R-value        & AUC            & R-value        & AUC            & R-value        & AUC            & R-value        & AUC            \\ \hline\hline

Resnet18                  & 0.759          & 0.875          & 0.799          & 0.863          & 0.774          & 0.852          & 0.717          & 0.840          & 0.762          & 0.858          \\ \hline
Resnet34                  & 0.787          & 0.903          & 0.787          & 0.866          & 0.768          & 0.887          & 0.723          & 0.861          & 0.766          & 0.879          \\ \hline
Resnet50                  & 0.799          & 0.894          & 0.823          & 0.888          & 0.795          & 0.880          & 0.741          & 0.858          & 0.789          & 0.880          \\ \hline
Vgg11                     & 0.843          & 0.919          & 0.838          & \textbf{0.916} & \textbf{0.832} & 0.917          & 0.772          & 0.881          & 0.821          & 0.908          \\ \hline
Vgg16                     & \textbf{0.865} & \textbf{0.923} & \textbf{0.863} & 0.913          & 0.824          & \textbf{0.918} & \textbf{0.804} & \textbf{0.901} & \textbf{0.839} & \textbf{0.914} \\ \hline
\end{tabular}





==> tables/patientLevelClassification.tex <==
\scriptsize


\begin{tabular}{|c|c|c|c|c|}
\hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}T-score\\ Thresholds\end{tabular}} & \multicolumn{2}{c|}{Osteoporosis} & \multicolumn{2}{c|}{Osteopenia} \\\cline{2-5}
& Sens            & Spec           & Sens           & Spec          \\\hline
-1.75                                                                         & 0.933           & 0.873          & 0.453          & 0.995         \\\hline
-2                                                                            & 0.844           & 0.929          & 0.341          & 0.998         \\\hline
-2.25                                                                         & 0.736           & 0.966          & 0.255          & 0.999         \\\hline
Flex                                                                          & 0.895           & 0.906          & 0.392          & 0.997        \\\hline
\end{tabular}


% \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
% \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}T-score\\ Thresholds\end{tabular}} & \multicolumn{2}{c|}{L1} & \multicolumn{2}{c|}{L2} & \multicolumn{2}{c|}{L3} & \multicolumn{2}{c|}{L4} & \multicolumn{2}{c|}{Average} \\\cline{2-11}
% & Sens       & Spec      & Sens       & Spec      & Sens       & Spec      & Sens       & Spec      & Sens         & Spec         \\\hline
% -1.75                                                                         & 93.9\%     & 85.1\%    & 91.7\%     & 89.1\%    & 93.4\%     & 91.1\%    & 85.0\%     & 93.1\%    & 91.0\%       & 89.6\%       \\\hline
% -2                                                                            & 86.2\%     & 91.0\%    & 85.0\%     & 93.0\%    & 84.8\%     & 94.8\%    & 75.4\%     & 95.4\%    & 82.8\%       & 93.6\%       \\\hline
% -2.25                                                                         & 77.6\%     & 95.3\%    & 76.3\%     & 95.8\%    & 72.0\%     & 96.9\%    & 68.9\%     & 97.4\%    & 73.7\%       & 96.4\%       \\\hline
% -2.5                                                                          & 61.9\%     & 97.5\%    & 63.5\%     & 97.9\%    & 60.7\%     & 98.3\%    & 54.5\%     & 98.9\%    & 60.2\%       & 98.1\%       \\\hline
% Flex                                                                          & 79.8\%     & 94.7\%    & 82.3\%     & 94.4\%    & 84.8\%     & 94.8\%    & 78.4\%     & 94.4\%    & 81.3\%       & 94.6\% \\ \hline
% \end{tabular}





==> tables/std.tex <==
\scriptsize
\begin{tabular}{|c|c|c|c|}
\hline
\multirow{2}{*}{Model} & \multicolumn{3}{c|}{L1$\sim$L4   Average} \\\cline{2-4} 
                       & STD         & ESTD        & p-value      \\\hline
Base                   & 0.129       & 0.086       & 0            \\\hline
MultiPatch             & 0.141       & 0.083       & 0.747        \\\hline
AttenMultiPatch        & 0.142       & 0.08        & 0.725        \\\hline
MultiROI               & 0.143       & 0.081       & 0.813        \\\hline
Proposed               & 0.144       & 0.077       & 0.778       \\\hline
\end{tabular}

% \multirow{2}{*}{Model} & \multicolumn{3}{c|}{L1} & \multicolumn{3}{c|}{L2} & \multicolumn{3}{c|}{L3} & \multicolumn{3}{c|}{L4} & \multicolumn{3}{c|}{Average} \\\cline{2-16} 
%                        & R-Val  & RMSE  & AUC   & R-Val  & RMSE  & AUC   & R-Val  & RMSE  & AUC   & R-Val  & RMSE  & AUC   & R-Val   & RMSE    & AUC     \\\hline
% Base                   & 0.859  & 0.089 & 0.952 & 0.87   & 0.101 & 0.96  & 0.86   & 0.104 & 0.966 & 0.823  & 0.12  & 0.963 & 0.853   & 0.104   & 0.96    \\\hline
% MultiPatch             & 0.873  & 0.071 & 0.958 & 0.877  & 0.08  & 0.967 & 0.873  & 0.083 & 0.971 & 0.834  & 0.098 & 0.965 & 0.864   & 0.083   & 0.965   \\\hline
% AttMultiPatch          & 0.885          & 0.068          & 0.964          & 0.888          & 0.076          & \textbf{0.967} & 0.882          & 0.081          & 0.969          & 0.846          & 0.094          & 0.964          & 0.875          & 0.08           & 0.966          \\\hline
% MultiROI               & 0.883  & 0.068 & 0.959 & 0.887  & 0.076 & 0.966 & 0.879  & 0.082 & 0.972 & 0.837  & 0.097 & 0.966 & 0.871   & 0.081   & 0.966   \\\hline
% \textbf{Proposed}      & \textbf{0.894} & \textbf{0.065} & \textbf{0.964} & \textbf{0.899} & \textbf{0.073} & 0.966          & \textbf{0.887} & \textbf{0.079} & \textbf{0.972} & \textbf{0.855} & \textbf{0.092} & \textbf{0.968} & \textbf{0.884} & \textbf{0.077} & \textbf{0.968} \\\hline


% \end{tabular}




